Improving Efficiency in Neural Network Accelerator Using Operands Hamming Distance optimization

Neural network accelerator is a key enabler for the on-device AI inference, for which energy efficiency is an important metric. The data-path energy, including the computation energy and the data movement energy among the arithmetic units, claims a significant part of the total accelerator energy. By revisiting the basic physics of the arithmetic logic circuits, we show that the data-path energy is highly correlated with the bit flips when streaming the input operands into the arithmetic units, defined as the hamming distance of the input operand matrices. Based on the insight, we propose a post-training optimization algorithm and a hamming-distance-aware training algorithm to co-design and co-optimize the accelerator and the network synergistically. The experimental results based on post-layout simulation with MobileNetV2 demonstrate on average 2.85X data-path energy reduction and up to 8.51X data-path energy reduction for certain layers.

==> doc/backup.tex <==

\begin{comment}
\subsection{Energy consumption in digital circuits}
\label{subsec:energy_consumption}



Here we first review the physics and see how energy is consumed in a digital circuit. Essentially, digital circuits are composed of PMOS/NMOS transistors and capacitance loading (as shown in the inverter example of Fig. 1). For datapath, energy consumption can be divided into three parts \cite{Rabaey:2008}
:
\begin{itemize}
    \item Switching: 0/1 states in digital circuit is physically represented by charged/discharged capacitor. When output or internal state changes from 0 to 1 or from 1 to 0 (bit flip), capacitor needs to be charged/discharged, which comes with an energy cost of $CV^{2}/2$ dissipated in resistance of PMOS/NMOS transistor.
    \item Glitch: when bit flips happens at input of PMOS/NMOS, PMOS and NMOS transistors are simultaneously turned on for a short period, which causes short-circuit current and consumes energy.
    \item Leakage: when transistors are turned off in steady state, there is still a small leakage current in transistors. Leakage contribution to energy in datapath is orders of magnitude smaller than glitch/switching contribution and can be ignored.
\end{itemize}
According to previous analysis, energy consumption in data path is mainly due to bit flip.
\begin{figure}[htp]
    \centering
    \includegraphics[width=4cm]{figs/CMOS_inverter_crop.pdf}
    \caption{Basic inverter circuit}
    \label{fig:inverter}
\end{figure}

\subsection{Systolic Array and Spatial Accelerator}
\label{subsec:systolic_array}


\meng{Need to add more description for systolic arrays (also, add necessary references) and also how to map a convolution layer or a matrix multiplication layer to the array.}
Systolic array is a highly efficient hardware implementation for neural network accelerator [Ref TPU]. In systolic array, an array of processing elements (PE) are tightly coupled. Input data flow spatially through the whole array, and each PE inside array works in a fully parallel manner.

\\Popular neural network layers, such as convolution layer and fully-connected layer, can be mapped to matrix multiplication and accelerated by systolic array. Fully-connected layer can be naturally described by input activation (column) vector $X$ multiplied by weight matrix $W$, where i-th row in $w$ corresponds to the weight for the i-th output activation. When mapped to systolic array, we can prefill array with $X$ and let $W$ flow through array, as shown in Example \ref{exg:matrix_vector}. 

\begin{example}
\label{exg:matrix_vector}

Consider a matrix-vector multiplier as an example: we have a data vector $X$ multiplied by weight matrix $W$, and output is a vector $Y$:
\begin{align*}
\begin{bmatrix}
W_{00} & W_{01}  &\dots & W_{0n} \\ 
W_{10} & W_{11}  &\dots & W_{1n}\\ 
\vdots & \vdots  & \ddots & \vdots \\ 
W_{m0} & W_{m1}  &\dots & W_{mn} 
\end{bmatrix} \cdot
\begin{bmatrix}
X_{0} \\ 
X_{1} \\ 
\vdots \\ 
X_{n} 
\end{bmatrix} =
\begin{bmatrix}
Y_{0} \\ 
Y_{1} \\ 
\vdots \\ 
Y_{m} 
\end{bmatrix}
\end{align*}
We can map this operation to a mini systolic array with single column. The column is pre-filled with X, and each time we pass one row of W. The operation of the array is shown in Fig. \ref{fig:1-col-array}.
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/1-col-array_crop.pdf}
    \caption{Single column array with pre-filled $X$ and multiplies with one row of $W$ per cycle}
    \label{fig:1-col-array}
\end{figure}

\end{example}

Similarly, convolutional layer can be mapped into matrix-matrix multiplication and accelrated by systolic array (Example ). The 3D weight kernel tensor can be unfolded into 2D weight matrix $W$ where $(Z_{in}, K_x, K_y)$ for each output channel is unfolded into one row of weight matrix $W$, while different rows in $W$ corresponds to different output channels $Z_{out}$. In addition, 3D input tensor can be unfolded into 2D input matrix $X$ and filled into each column of array, and convolution operation can be equivalently implemented by matrix-matrix multiplication $W*X$.

\begin{example}
\label{exg:matrix_matrix}

Consider a matrix-matrix multiplication as an example: we have an input matrix $X$ multiplied by weight matrix $W$, and output is matrix $Y$:
\begin{align*}
\begin{bmatrix}
W_{00} &\dots & W_{0n} \\ 
W_{10} &\dots & W_{1n}\\ 
\vdots & \ddots & \vdots \\ 
W_{m0} &\dots & W_{mn} 
\end{bmatrix} \cdot
\begin{bmatrix}
X_{00}  &\dots & X_{0k} \\ 
X_{10}  &\dots & X_{1k}\\ 
\vdots  & \ddots & \vdots \\ 
X_{n0}  &\dots & X_{mk} 
\end{bmatrix} =
\begin{bmatrix}
Y_{00} &\dots & Y_{0k} \\ 
Y_{10} &\dots & Y_{1k}\\ 
\vdots & \ddots & \vdots \\ 
Y_{m0} &\dots & Y_{mk} 
\end{bmatrix}
\end{align*}
We can map this operation to a multi-column systolic array. The array is pre-filled with $X$, then each time we send one row of $W$ into array and get one row of output $Y$. The operation of the array is shown in Fig. \ref{fig:mul-col-array}.
\end{example}
\end{comment}




which confirms the relation between the bit flips and the datapath energy. 

Consider the example with the following weight matrix: 
\begin{equation*}
W=\begin{bmatrix}
0000 & 0000  &0000 & 0000 \\ 
1111 & 1111  &1111 & 1111 \\ 
0000 & 0000  &0000 & 0000 \\ 
1111 & 1111  &1111 & 1111
\end{bmatrix} 
= \begin{bmatrix}
W_{0}\\
W_{1}\\
W_{2}\\
W_{3}
\end{bmatrix}.
\end{equation*}
Without loss of generality, we assume multiplication is based on 4-bit operands. If we send row vectors of W into array with the sequence of $(W_{0},W_{1},W_{2},W_{3})$ (i.e., [0000 0000 0000 0000], [1111 1111 1111 1111], [0000 0000 0000 0000], [1111 1111 1111 1111]) and save output to the accumulation buffer entry at (0,1,2,3), then the bit flipping for each multiplier is $4 (0000\rightarrow 1111) + 4 (1111\rightarrow 0000) + 4 (0000\rightarrow 1111) = 12$ and total multiplier bit flipping is 48. On the other hand, if we send row vectors of W into array with the sequence of $(W_{0},W_{2},W_{1},W_{3})$ (i.e., [0000 0000 0000 0000], [0000 0000 0000 0000], [1111 1111 1111 1111], [1111 1111 1111 1111]) and save output to memory address at (0,2,1,3), then we can achieve exactly the same function as the first case but the bit flipping for each multiplier is $0 (0000\rightarrow 0000) + 4 (0000\rightarrow 1111) + 0 (1111\rightarrow 1111) = 4$ and total multiplier bit flipping is 16, which is 1/3 compared with the original sequence. This means we can improve energy consumption in multiplier by roughly 3X by simply optimizing the weight feeding sequence.

In coding theory, the bit flips between two bit strings are defined as the Hamming distance between two numbers. We define the total Hamming Distance (THD) of the weight sequence as the sum of Hamming distance between neighboring weight bit strings in the sequence. 

\begin{example}
\label{exg:THD_bitflip}

Without loss of generality, we assume multiplication is based on 4-bit operands. For illustration, let 
\begin{align*}
W=\begin{bmatrix}
0000 & 0000  &0000 & 0000 \\ 
1111 & 1111  &1111 & 1111\\ 
0000 & 0000  &0000 & 0000 \\ 
1111 & 1111  &1111 & 1111
\end{bmatrix} =  \begin{bmatrix}
W_{0}\\
W_{1}\\
W_{2}\\
W_{3}
\end{bmatrix},
X=\begin{bmatrix}
0001 \\ 
0001 \\ 
0001 \\ 
0001 
\end{bmatrix}
\end{align*}
If we send row vectors of W into array with the sequence of $(W_{0},W_{1},W_{2},W_{3})$ (i.e., [0000 0000 0000 0000], [1111 1111 1111 1111], [0000 0000 0000 0000], [1111 1111 1111 1111]) and save output to memory address at (0,1,2,3), then the bit flipping for each multiplier is $4 (0000\rightarrow 1111) + 4 (1111\rightarrow 0000) + 4 (0000\rightarrow 1111) = 12$ and total multiplier bit flipping is 48. On the other hand, if we send row vectors of W into array with the sequence of $(W_{0},W_{2},W_{1},W_{3})$ (i.e., [0000 0000 0000 0000], [0000 0000 0000 0000], [1111 1111 1111 1111], [1111 1111 1111 1111]) and save output to memory address at (0,2,1,3), then we can achieve exactly the same function as the first case but the bit flipping for each multiplier is $0 (0000\rightarrow 0000) + 4 (0000\rightarrow 1111) + 0 (1111\rightarrow 1111) = 4$ and total multiplier bit flipping is 16, which is 1/3 compared with the original sequence. This means we can improve energy consumption in multiplier by roughly 3X by simply optimizing weight feeding sequence.
\end{example}



\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/mul-col-array-crop.pdf}
    \caption{Multi-Column array with pre-filled $X$ and multiplies with one row of $W$ per cycle to implement matrix-matrix multiplication}
    \label{fig:mul-col-array}
\end{figure}

\\In coding theory, Hamming distance $H(a,b)$ between two bit strings is defined as the number of positions at which the corresponding bits are different \cite{Hamming:1950}. For input/weight-array, we can define total Hamming distance as the sum of Hamming distances between neighboring weight/input bit strings in the sequence. For sequence of $(00,01,10,11)$, the total Hamming distance, $THD(00,01,10,11)=H(00,01) + H(01,10) + H(10,11) = 1+2+1 = 4$. In the previous example, the bit strings for weight sequence of  $(W_{0},W_{1},W_{2},W_{3})$ = $([0000 0000 0000 0000], [1111 1111 1111 1111],$ $[0000 0000 0000 0000], [1111 1111 1111 1111])$  is $(0000000000000000, 1111111111111111,$ $0000000000000000,1111111111111111)$ and total Hamming distance is 48. On the other hand, the bit strings for weight sequence of  $(W_{0},W_{2},W_{1},W_{3})$  is $(0000000000000000, 0000000000000000,$ $1111111111111111, 1111111111111111)$ and total Hamming distance is 12. 

\\THD and datapath energy are strongly correlated. In order to verify this correlation, we designed an input stationary systolic array with 8 rows and 2 columns. Each cell in array can natively support 8-bit x 4-bit multiplication, where 8-bit is for CNN model input activation matrix ($X$) and 4-bit is for model weight matrix ($W$). The array is synthesized using Design Compiler and place & route using IC Compiler II with TSMC 7nm ULVT technology, and can meet 1GHz timing constraint. The cycle-accurate post layout power is extracted by Prime Time PX, and converted into energy by multiplying total operation cycle time. We generated random weight data sequences with various length, and collected data of THD and energy consumption of the array. As shown in Fig.\ref{fig:THD_energy}, strong correlation is observed between THD and energy consumption. 




\begin{algorithm}[tb]
   \caption{Greedy search for TSP}
   \label{alg:example}
\begin{algorithmic}
   \STATE {\bfseries Input:} list $A[n]$ 
   \STATE {\bfseries Output:} optimized sequence $S[n]$ 
   \STATE $S[0] = A[0]$
   \STATE remove $A[0]$ from $A$
   \FOR{$i=1$ {\bfseries to} $n-1$}
   \STATE$j=argmin(H(S[i-1],A[j]))$
   \STATE $S[i] = A[j]$
   \STATE remove $A[j]$ from $A$
   \ENDFOR
\end{algorithmic}
\end{algorithm}


such that each output channel has to exist and only exist once in $S$.

Consider the matrix multiplication operation in systolic array to accelerate neural network computation. Inspired by Example \ref{exg:THD_bitflip}, we can reorder the sequence of matrix feeding into array to minimize THD and therefore energy consumption. The straightforward case will be input-stationary array where layer input is pre-filled into array PE and we can adjust how the rows of $W$ are fed into array to minimize THD. As discussed in Example \ref{exg:matrix_matrix}, each row in $W$ matrix corresponds to one output channel of neural network, thus this optimization is essentially just adjusting the order of output channels when doing compute for minimal THD and there is no influence in terms of neural network functionality. It should also be noted that plain output channel reordering is fully in model level and does not involve any hardware overhead.
%We describe how to apply the Hamming distance optimization technique to accelerator array targeting convolutional neural network (CNN). CNN operation can be unrolled into matrix-matrix multiplication, so we can use a multi-column systolic array to accelerate CNN. 

\\Formally, let's assume we have an input list of $W={W_1,W_2,...,W_n}$ with size $n$, where each element $W_i$ is a bit string of length $l$. $W$ is then fed into array with sequence $S = (W_{s_1},W_{s_2},...,W_{s_n})$ where $s_i\in[1,n]$ and $s_j\neq s_k$ if $j\neq k$. This way we guarantee all elements of $W$ are fed into array only once. The problem is to find the best sequence $S_b$ with smallest $THD(S_b)$.

\\In the case of matrix-matrix multiplication for neural network acceleration, the sequence size $n$ equals to the number of output channels, and bit string is just each row vector of $W$ and its length $l$ equals to $K_x*K_y*Z_{in}*Bit\_Width$, where $K_x$, $K_y$ are kernel size in (x,y) plane, $Z_{in}$ is the number of input channels and $Bit\_Width$ is the number of bits input data representation after quantization. 

\meng{Need to mention that no extra hardware support is needed}

\meng{Need to mention the main problems with the greedy approach and motivate the clustering and segment algorithm as well as the training-aware regularization}

This is actually a Traveling Salesperson Problem (TSP). Each $Ai$ in $A$ is one location to visit, Hamming distance $H(A_j,A_k)$ is the distance between two locations and we want to find an optimized sequence to visit those locations with the minimal $THD$. Exhaustive search algorithm for size n has time complexity of $O(n!)$, and is not feasible for real world cases. Fortunately, greedy search can also achieve decent results on TSP (cite TODO). The pseudo code for greedy search can be described in Algorithm 1:
% \subsubsection{Naive greedy search and its mapping to hardware}

In order to evaluate the effectiveness of greedy-search-based output channel reordering, we trained a MobileNet V2 network [ref TODO] with CIFAR100 datset and quantize its weight into 4-bit. Since pointwise convolution layers occupy more than 95\% of total computational load in MobileNet V2, we focus on optimizing pointwise convolution layers. The pointwise layer weight dimension is summarized in Table~\ref{table-mbnetv2}. Table~\ref{table-plain-greedy} is a summary of typical layers in the network and Hamming distances with greedy search. With similar $l$ (e.g., layer[7] and layer[28]), THD improvement increases with larger $n$. With increased $l$, however, the obtainable THD improvement decreases sharply.

\begin{table*}[t]
\caption{Pointwise Convolution Layers for MobileNet V2.}
\label{table-mbnetv2}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm}}
%\begin{tabular}{l c c c c c c r}
\toprule
Pointwise layer \# & weight dimension & Pointwise layer \# & weight dimension & Pointwise layer \# & weight dimension  \\        
\midrule
0     & (16,32)   &12 &(64,192) &24 &(96,576)        \\
1     & (96,16)   &13 &(384,64) &25 &(576,96)         \\
2     & (24,96)   &14 &(64,384) &26 &(160,576)      \\
3     & (144,24)  &15 &(384,64) &27 &(960,160)         \\
4     & (24,144)  &16 &(64,384) &28 &(160,960)       \\
5     & (144,24)  &17 &(384,64) &29 &(960,160)       \\
6     & (32,144)  &18 &(64,384) &30 &(160,960)        \\
7     & (192,32)  &19 &(384,64) &31 &(960,160)         \\
8     & (32,192)  &20 &(96,384) &32 &(320,960)      \\
9     & (192,32)  &21 &(576,96) &33 &(1280,320)         \\
10    & (32,192)  &22 &(96,576) &  &       \\
11    & (192,32)  &23 &(576,96) &  &       \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\begin{table*}[t]
\caption{Hamming Distance Improvement with Various $n$ and $l$.}
\label{table-plain-greedy}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm}}
%\begin{tabular}{l c c c c c c r}
\toprule
layer & sequence size ($n$) & bit string length ($l$) & THD w/o optimization ($THD_{S_u}$) & THD with greedy search ($THD_{S_b}$) & $\frac{THD_{S_u}}{THD_{S_b}}$ \\        
\midrule
layer{[}7{]}     & 192                   & 32*4                           & 12034                                  & 7820                                & 1.54          \\
layer{[}8{]}     & 32                    & 192*4                          & 11026                                  & 9368                               & 1.18           \\
layer{[}15{]}     & 384                   & 64*4                           & 48399                                  & 36337                               & 1.33          \\
layer{[}16{]}     & 64                    & 384*4                          & 46511                                  & 42594                               & 1.09         \\
layer{[}21{]}     & 576                   & 96*4                           & 108510                                 & 85199                              & 1.27         \\
layer{[}22{]}     & 96                    & 576*4                          & 108421                                  & 100332                              & 1.08        \\
layer{[}27{]}     & 960                   & 160*4                          & 299936                                 & 255221                            & 1.18         \\
layer{[}28{]}     & 160                   & 960*4                          & 302390                                 & 286703                             & 1.05         \\
layer{[}33{]}     & 1280                  & 320*4                          & 813519                                 & 670299                            & 1.21         \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

The challenge of Hamming distance optimization lies in large $l$. As can be seen from Table~\ref{table-1}, even with an aggressive 4-bit quantization, $l$ is still too large in most layers, which limits THD to less than 30\%. 

% \subsubsection{Improve optimization by segment-then-search}

\subsection{Input Channel Segmentation and Clustering}
\label{subsec:input_clustering}

\meng{Need to merge these the original draft and the c clustering write-up}
The THD optimization overhead induced by large $l$ can be solved by hardware-software co-design. The endeavor comes into two folds: input channel semgentation and input channel clustering.

\subsubsection{Input Channel Segmentation}
In order to reduce $l$ in THD optimization, we can segment weight matrix $W$ with large $l$ into several small sub-matrices $W'$. The row (output channel) count of each $W'$ is the same as $W$ (so the sequence length $n$ keeps unchanged), while the column (input channel) count of each $W'$ is just a fraction of $W$ to reduce $l$; then, we can perform greedy search on each $W'$ to optimize THD (segment-then-optimize greedy search, STOGS). Since $W'$ has smaller $l$ than $W$, better THD optimization improvement can be achieved. When doing computation, we send one row of $W'$ into array each time, and merge partial sums generated from each $W'$ to get final output.

\\This segment also makes sense from hardware perspective. When we have a $W$ with more column count than the array can accommodate at one time, segment of $W$ into multiple sub-matrices $W'$ and then merge final output is required regardless. The only difference is the address mapping part - when we have regular segment, the $i$-th row in each sub-matrix $W'$ always corresponds to the same output channel stored in address $i$; when we have STOGS, the $i$-th row in different $W'$ may corresponds to different output channel and therefore should be stored into different output addresses. The detailed hardware support needed is discussed in Section \ref{sec:hw_sup}.



%Take MobileNet V2 layer[12] as an example. This layer is a pointwise convolution layer with convolution kernel size 1x1, input channel 32 and output channel 192. Therefore the weight matrix W has 192 rows and 32 columns, and can be represented as $W[0:191][0:31]$. One row of $W$ with 32 elements is supposed to be fed into accelerator array for matrix multiplication. But what if the accelerator only has 8 multiplier elements in one column, and so cannot accommodate 32 elements of a full row from $W$? Then naive way is to segment $W$ into multiple sub-matrices and send one row of such sub-matrix into array. For example, we can segment W into four sub-matrices, with $W_0 = W[0:191][0:7]$, $W_1 = W[0:191][8:15]$, $W_2 = W[0:191][16:23]$, $W_3 = W[0:191][24:31]$. We do $W_0$ computation first, save partial sum into memory, and send $W_1$ next, add partial sum to the corresponding memory location, etc. When we apply optimization first, we apply to rows of $W$, and get a new weight matrix $W’$ with optimized row sequence, then segment $W'$ into $W'_0$, $W'_1$, $W'_2$, $W'_3$ and send into array. When doing optimize-then-segment (OTS), the $l$ for greedy search remains the same regardless of segment or not, so large $l$ issue also remains.

%Segment-then-optimize (STO) can overcome this issue. In this scheme, we first segment $W$ into $W_0$, $W_1$, $W_2$, $W_3$ as described in the previous paragraph, then optimize $W_0$, $W_1$, $W_2$ and $W_3$ independently. In this case, each $W_0$, $W_1$, $W_2$ and $W_3$ has 8 elements (instead of 32) in one row, and so its effective bit string length $l$ is 8*4 = 32 instead of 128. On the other hand, the number of rows in $W_0$, $W_1$, $W_2$ and $W_3$ is still 192 (for simplicity here we are assuming the output buffer memory is deep enough to accommodate 192 entries), so the sequence size $n$ is unchanged. With segment-then-optimize, effective $l$ is decoupled from layer size, therefore the optimized THD ($THD_{S_{b,sto}}$) is much smaller than previous $THD_{S_b}$ as shown in Table~\ref{table-2} for most layers. With STO scheme, we can achieve 1.5-2.5X THD improvement in average case for 1x1 pointwise convolution layers in MobileNet V2, which occupies more than 95\% of total operations in MobileNet V2.
The STOSG result is shown in Table \ref{table-2}. As can be seen, the with STOSG, we can achieve 1.5-2.5X THD improvement in average case for 1x1 pointwise convolution layers in MobileNet V2, which occupies more than 95\% of total operations. 
\begin{table*}[t]
\caption{Hamming Distance Improvement with Optimize-Then-Segment and segment-Then-Optimize.}
\label{table-2}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm} m{1.5cm}}
%\begin{tabular}{l c c c c c c r}
\toprule
layer & sequence size ($n$) & bit string length $l$ for OTS & bit string length $l$ for STO & THD w/o optimization ($THD_{S_u}$) & THD with OTS ($THD_{S_{OTS}}$)  & THD with OTS ($THD_{S_{STO}}$) & $\frac{THD_{S_{u}}}{THD_{S_{STO}}}$ \\        
\midrule
layer{[}12{]}     & 192                   & 32*4          &8*4                 & 11145                                  & 8247 &\textbf{5536}                                & \textbf{2.01319}          \\
layer{[}14{]}     & 32                    & 192*4         &8*4                & 10774                                  & 10088 &\textbf{6998}                                & \textbf{1.53958}           \\
layer{[}21{]}     & 384                   & 64*4          &8*4                 & 44876                                  & 35993 &\textbf{20677}                              & \textbf{2.17033}          \\
layer{[}23{]}     & 64                    & 384*4         &8*4                 & 44542                                  & 41620   &\textbf{26211}                            & \textbf{1.69936}         \\
layer{[}33{]}     & 576                   & 96*4          &8*4                 & 101142                                 & 83671   &\textbf{43947}                           &\textbf{2.30145}          \\
layer{[}35{]}     & 96                    & 576*4         &8*4                 & 98727                                  & 93718   &\textbf{55294}                            &\textbf{1.78549}         \\
layer{[}42{]}     & 960                   & 160*4         &8*4                  & 282821                                 & 243642 &\textbf{115806}                            &\textbf{2.4422}          \\
layer{[}44{]}     & 160                   & 960*4         &8*4                 & 278012                                 & 266285  &\textbf{143794}                            &\textbf{1.9334}          \\
layer{[}51{]}     & 1280                  & 320*4         &8*4                   & 765310                                 & 690579 &\textbf{309417}                           &\textbf{2.47339}          \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}




To sum up, the STOSG scheme greatly improves the effect of Hamming distance optimization in real world neural network models. Given total number of PE cells in one systolic array, STOSG scheme prefers a “flat” aspect ratio; i.e., more columns and fewer rows in systolic array to reduce l in each segment. With row number of 8, we can achieve 1.5-2.5X THD improvement in pointwise convolution layers in MobileNet V2. 

However, the aspect ratio of systolic array is also constrained by other considerations. With more number of columns in input-stationary systolic array, it takes more pixels in x-y plane to fill the whole array. This is not a problem for small-scale arrays with low total PE counts, however it may induce utilization issue for large array as it needs more pixels to fill up columns, especially for deep layers with small x-y size but with deep $Z_{in}$. This is where c clustering comes into play.

\subsubsection{Input Channel Clustering}
\input{doc/c_clustering}


Usually, the activations are packed along the channel direction or the spatial direction into words and then, stored in the global buffer. If the activations are packed along the spatial direction, the impact of input channel clustering is negligible except for a change of the input address generation sequence


There are mainly two commonly used memory layouts for the activations: 1) activations are packed along the spatial direction into words and stored in the global buffer; and 2) activations are packed along the channel direction into words and stored in the global buffer.


To support segment-then-reorder algorithm, specific hardware blocks are needed.

The hardware overhead to support segment-then-optimize greedy search (STOGS) is minimal. in STOGS scheme, the same row in different segmented sub-matrices $W^\prime$ may correspond to partial sum of different output channels, which is detailed in Example \ref{exg:STOSG}. In order to make sure correct reduction of partial sums and keep the same computation result as original neural network, we need to add one extra memory address trace controller in hardware to guide the partial sum reduction.

\begin{example}
\label{exg:STOSG}
As an illustrative example, assume $W$ is a 4x4 matrix and we want to do matrix-vector multiplication:
$$\begin{bmatrix}
W_{00} & W_{01}  &W_{02} &W_{03} \\ 
W_{10} & W_{11}  &W_{12} &W_{13}\\ 
W_{20} & W_{21}  &W_{22} &W_{23} \\ 
W_{30} & W_{31}  &W_{32} &W_{33}
\end{bmatrix} *  \begin{bmatrix}
X_{0}\\
X_{1}\\
X_{2}\\
X_{3}
\end{bmatrix} = \begin{bmatrix}
Y_{0}\\
Y_{1}\\
Y_{2}\\
Y_{3}
\end{bmatrix}
$$
The memory layout for $Y$ is $Y_0$ in memory address 0, $Y_1$ in address 1, $Y_2$ in address 2 and $Y_3$ in address 3. Therefore $W$ has the first row $[W_{00}\; W_{01}\;  W_{02}\; W_{03}]$ corresponds to $Y_0$ at memory address 0, second row $[W_{10}\;  W_{11}\;  W_{12}\;  W_{13}]$ corresponds to $Y_1$ at memory address 1, the third row $[W_{20}\;  W_{21}\;  W_{22}\;  W_{23}]$ corresponds to $Y_2$ at memory address 2, and the fourth row $[W_{30}\;  W_{31}\;  W_{32}\;  W_{33}]$ corresponds to $Y_3$ at memory address 3. Further assume we segment $W$ into two sub-matrices $W_0$ and $W_1$ each with two columns:
$$W_0=\begin{bmatrix}
W_{00} & W_{01}  \\ 
W_{10} & W_{11} \\ 
W_{20} & W_{21}  \\ 
W_{30} & W_{31} 
\end{bmatrix} , W_1 = \begin{bmatrix}
W_{02} &W_{03} \\ 
W_{12} &W_{13}\\ 
W_{22} &W_{23} \\ 
W_{32} &W_{33}
\end{bmatrix} 
$$
For $W_0$, the first row $[W_{00}\; W_{01}]$ corresponds to partial sum of $Y_0$ at memory address 0, second row $[W_{10}\; W_{11}]$ corresponds to partial sum of $Y_1$ at memory address 1, the third row $[W_{20}\; W_{21}]$ corresponds to partial sum of $Y_2$ at memory address 2, and the fourth row $[W_{30}\; W_{31}]$ corresponds to partial sum of $Y_3$ at memory address 3. For $W_1$, the first row $[W_{02}\; W_{03}]$ corresponds to partial sum of $Y_0$ at memory address 0, second row $[W_{12}\; W_{13}]$ corresponds to partial sum of $Y_1$ at memory address 1, the third row $[W_{22}\; W_{23}]$ corresponds to partial sum of $Y_2$ at memory address 2, and the fourth row $[W_{32}\; W_{33}]$ corresponds to partial sum of $Y_3$ at memory address 3. 

After optimization, assume we have:
$$W'_0=\begin{bmatrix}
W_{00} & W_{01}  \\ 
W_{20} & W_{21} \\ 
W_{10} & W_{11}  \\ 
W_{30} & W_{31} 
\end{bmatrix} , W'_1 = \begin{bmatrix}
W_{02} &W_{03} \\ 
W_{22} &W_{23}\\ 
W_{12} &W_{13} \\ 
W_{32} &W_{33}
\end{bmatrix} 
$$
For $W'_0$, the first row $[W_{00}\; W_{01}]$ corresponds to partial sum of $Y_0$ at memory address 0, second row $[W_{20}\; W_{21}]$ corresponds to partial sum of $Y_2$ at memory address 2, the third row $[W_{10}\; W_{11}]$ corresponds to partial sum of $Y_1$ at memory address 1, and the fourth row $[W_{30}\; W_{31}]$ corresponds to partial sum of $Y_3$ at memory address 3. For $W'_1$, the first row $[W_{22}\; W_{23}]$ corresponds to partial sum of $Y_3$ at memory address 3, second row $[W_{12} W_{13}]$ corresponds to partial sum of $Y_1$ at memory address 1, the third row $[W_{22}\; W_{23}]$ corresponds to partial sum of $Y_2$ at memory address 2, and the fourth row $[W_{02}\; W_{03}]$ corresponds to partial sum of $Y_0$ at memory address 0. Therefore when feeding $W'_0$ and $W'_1$ into array, the memory trace for output partial sum storage is different (see Fig.~\ref{fig:Array_mem_mapping}).
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/mem_array_crop.pdf}
    \caption{Array mapping for STOSG}
    \label{fig:Array_mem_mapping}
\end{figure}
\end{example}

The various output memory trace for different optimized sub-matrix can be controlled by a simple SRAM-based look-up table (LUT), as shown in Fig. \ref{fig:overhead_sto}. With output buffer depth of $D$, the LUT needs to have at least $D$ entries and each entry should have $log_2D$ bits. For reasonable output buffer depth (\<1024), the LUT SRAM size is less than 2KB. Therefore segment-then-optimize has very limited energy and area overhead.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/overhead_segment_crop.pdf}
    \caption{Diagram for integrating array and memory system with output memory trace LUT to support segment-then-optimize}
    \label{fig:overhead_sto}
\end{figure}
%Another concern may be whether sequence size n can be limited by output memory depth. 

\\The finite size of output buffer can also influence segment scheme. In computation, different rows of sub-matrices $W'$ are sent into array once each time, and the partial sum of each row is stored in a different entry in output buffer. The size of output buffer defines how many rows of the same $W'$ can be sent into array without further partial sum reduce and/or memory write out. When the number of rows of $W'$ is larger than output buffer size, we will need to further segment row of $W'$. This row segment does not effect STOGS optimization, as shown in Example \ref{exg:output_buffer}.
\begin{example}
\label{exg:output_buffer}
Take the MobileNet V2 layer[7] case, where each optimized sub-matrix $W'_0,W'_1,W'_2$ and $W'_3$ has 192 rows. Assume we only have output memory depth of 64, then we will need to do reduction and output buffer write out when we send 64 rows, so $W'_0,W'_1,W'_2$ and $W'_3$ will be sent in an interleaving manner. In other words, instead of directly sending $W'_0[0:191][0:7]$ then  $W'_1[0:191][8:15]$ then $W'_2[0:191][16:23]$ then $W'_3[0:191][24:31]$ the do output buffer write out, we will need to send with the sequence of $W'_0[0:63][0:7],\; W'_1[0:63][0:7],\; W'_2[0:63][0:7],\; W'_3[0:63][0:7]$, (do memory write out), $W'_0[64:127][0:7],\; W'_1[64:127][0:7],\; W'_2[64:127][0:7],\; W'_3[64:127][0:7]$, (do memory write out), $W'_0[128:191][0:7],\; W'_1[128:191][0:7],\; W'_2[128:191][0:7],\; W'_3[128:191][0:7]$, (do memory write out). After closer examination, this will have minimal impact on THD improvement. Comparing two cases, the only possible extra bit flipping happen when we switch among different sub-matrices; i.e., $W'_0[63][0:7]\rightarrow W'_1[0][0:7],\; W'_1[63][0:7]\rightarrow W'_2[0][0:7],\; W'_2[63][0:7]\rightarrow W'_3[0][0:7],\; W'_3[63][0:7]\rightarrow W'_0[64][0:7],\; W'_0[127][0:7]\rightarrow  W'_1[64][0:7],\; W'_1[127][0:7]\rightarrow W'_2[64][0:7],\; W'_2[127][0:7]\rightarrow W'_3[64][0:7],\; W'_3[127][0:7]\rightarrow W'_0[128][0:7],\; W'_0[191][0:7]\rightarrow W'_1[128][0:7],\; W'_0[191][0:7]\rightarrow W'_1[128][0:7],\; W'_1[191][0:7]\rightarrow W'_2[128][0:7],\; W'_2[191][0:7]\rightarrow W'_3[128][0:7]$. With output buffer depth of $d$, the extra bit flipping happens once after sending sequence length of d, and Hamming Distance overhead will be $\frac{1}{d}$. For reasonable d (e.g. 64 or 128), this overhead is less than 2\%.
\end{example}

Unlike STOSG, C clustering proposed in Section \ref{subsec:c_clustering} does not involve partial sum address issue. C clustering is essentially a dual process of output channel reordering, where output reordering reorders rows of weight matrix and C clustering reorders columns of weight matrix. This means that C clustering will only influence the memory fetching of input activation, but no hardware overhead is involved.

\label{sec:hardware_support}



In order to avoid any complication or modification to the input fetching logic, 

we propose to re-arrange the input activations of the current layer before it is stored 

\meng{Keep minimum impact to the rest of the system, reorder the output channels first before storing everything back to the memory. Reuse the memory address trace controller above.}


Usually, the activations are packed along the channel direction or the spatial direction into words and then, stored in the global buffer. If the activations are packed along the spatial direction, the impact of input channel clustering is negligible except for a change of the input address generation sequence


There are mainly two commonly used memory layouts for the activations: 1) activations are packed along the spatial direction into words and stored in the global buffer; and 2) activations are packed along the channel direction into words and stored in the global buffer.


To support segment-then-reorder algorithm, specific hardware blocks are needed.

The hardware overhead to support segment-then-optimize greedy search (STOGS) is minimal. in STOGS scheme, the same row in different segmented sub-matrices $W^\prime$ may correspond to partial sum of different output channels, which is detailed in Example \ref{exg:STOSG}. In order to make sure correct reduction of partial sums and keep the same computation result as original neural network, we need to add one extra memory address trace controller in hardware to guide the partial sum reduction.

\begin{example}
\label{exg:STOSG}
As an illustrative example, assume $W$ is a 4x4 matrix and we want to do matrix-vector multiplication:
$$\begin{bmatrix}
W_{00} & W_{01}  &W_{02} &W_{03} \\ 
W_{10} & W_{11}  &W_{12} &W_{13}\\ 
W_{20} & W_{21}  &W_{22} &W_{23} \\ 
W_{30} & W_{31}  &W_{32} &W_{33}
\end{bmatrix} *  \begin{bmatrix}
X_{0}\\
X_{1}\\
X_{2}\\
X_{3}
\end{bmatrix} = \begin{bmatrix}
Y_{0}\\
Y_{1}\\
Y_{2}\\
Y_{3}
\end{bmatrix}
$$
The memory layout for $Y$ is $Y_0$ in memory address 0, $Y_1$ in address 1, $Y_2$ in address 2 and $Y_3$ in address 3. Therefore $W$ has the first row $[W_{00}\; W_{01}\;  W_{02}\; W_{03}]$ corresponds to $Y_0$ at memory address 0, second row $[W_{10}\;  W_{11}\;  W_{12}\;  W_{13}]$ corresponds to $Y_1$ at memory address 1, the third row $[W_{20}\;  W_{21}\;  W_{22}\;  W_{23}]$ corresponds to $Y_2$ at memory address 2, and the fourth row $[W_{30}\;  W_{31}\;  W_{32}\;  W_{33}]$ corresponds to $Y_3$ at memory address 3. Further assume we segment $W$ into two sub-matrices $W_0$ and $W_1$ each with two columns:
$$W_0=\begin{bmatrix}
W_{00} & W_{01}  \\ 
W_{10} & W_{11} \\ 
W_{20} & W_{21}  \\ 
W_{30} & W_{31} 
\end{bmatrix} , W_1 = \begin{bmatrix}
W_{02} &W_{03} \\ 
W_{12} &W_{13}\\ 
W_{22} &W_{23} \\ 
W_{32} &W_{33}
\end{bmatrix} 
$$
For $W_0$, the first row $[W_{00}\; W_{01}]$ corresponds to partial sum of $Y_0$ at memory address 0, second row $[W_{10}\; W_{11}]$ corresponds to partial sum of $Y_1$ at memory address 1, the third row $[W_{20}\; W_{21}]$ corresponds to partial sum of $Y_2$ at memory address 2, and the fourth row $[W_{30}\; W_{31}]$ corresponds to partial sum of $Y_3$ at memory address 3. For $W_1$, the first row $[W_{02}\; W_{03}]$ corresponds to partial sum of $Y_0$ at memory address 0, second row $[W_{12}\; W_{13}]$ corresponds to partial sum of $Y_1$ at memory address 1, the third row $[W_{22}\; W_{23}]$ corresponds to partial sum of $Y_2$ at memory address 2, and the fourth row $[W_{32}\; W_{33}]$ corresponds to partial sum of $Y_3$ at memory address 3. 

After optimization, assume we have:
$$W'_0=\begin{bmatrix}
W_{00} & W_{01}  \\ 
W_{20} & W_{21} \\ 
W_{10} & W_{11}  \\ 
W_{30} & W_{31} 
\end{bmatrix} , W'_1 = \begin{bmatrix}
W_{02} &W_{03} \\ 
W_{22} &W_{23}\\ 
W_{12} &W_{13} \\ 
W_{32} &W_{33}
\end{bmatrix} 
$$
For $W'_0$, the first row $[W_{00}\; W_{01}]$ corresponds to partial sum of $Y_0$ at memory address 0, second row $[W_{20}\; W_{21}]$ corresponds to partial sum of $Y_2$ at memory address 2, the third row $[W_{10}\; W_{11}]$ corresponds to partial sum of $Y_1$ at memory address 1, and the fourth row $[W_{30}\; W_{31}]$ corresponds to partial sum of $Y_3$ at memory address 3. For $W'_1$, the first row $[W_{22}\; W_{23}]$ corresponds to partial sum of $Y_3$ at memory address 3, second row $[W_{12} W_{13}]$ corresponds to partial sum of $Y_1$ at memory address 1, the third row $[W_{22}\; W_{23}]$ corresponds to partial sum of $Y_2$ at memory address 2, and the fourth row $[W_{02}\; W_{03}]$ corresponds to partial sum of $Y_0$ at memory address 0. Therefore when feeding $W'_0$ and $W'_1$ into array, the memory trace for output partial sum storage is different (see Fig.~\ref{fig:Array_mem_mapping}).
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/mem_array_crop.pdf}
    \caption{Array mapping for STOSG}
    \label{fig:Array_mem_mapping}
\end{figure}
\end{example}

The various output memory trace for different optimized sub-matrix can be controlled by a simple SRAM-based look-up table (LUT), as shown in Fig. \ref{fig:overhead_sto}. With output buffer depth of $D$, the LUT needs to have at least $D$ entries and each entry should have $log_2D$ bits. For reasonable output buffer depth (\<1024), the LUT SRAM size is less than 2KB. Therefore segment-then-optimize has very limited energy and area overhead.
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/overhead_segment_crop.pdf}
    \caption{Diagram for integrating array and memory system with output memory trace LUT to support segment-then-optimize}
    \label{fig:overhead_sto}
\end{figure}
%Another concern may be whether sequence size n can be limited by output memory depth. 

\\The finite size of output buffer can also influence segment scheme. In computation, different rows of sub-matrices $W'$ are sent into array once each time, and the partial sum of each row is stored in a different entry in output buffer. The size of output buffer defines how many rows of the same $W'$ can be sent into array without further partial sum reduce and/or memory write out. When the number of rows of $W'$ is larger than output buffer size, we will need to further segment row of $W'$. This row segment does not effect STOGS optimization, as shown in Example \ref{exg:output_buffer}.
\begin{example}
\label{exg:output_buffer}
Take the MobileNet V2 layer[7] case, where each optimized sub-matrix $W'_0,W'_1,W'_2$ and $W'_3$ has 192 rows. Assume we only have output memory depth of 64, then we will need to do reduction and output buffer write out when we send 64 rows, so $W'_0,W'_1,W'_2$ and $W'_3$ will be sent in an interleaving manner. In other words, instead of directly sending $W'_0[0:191][0:7]$ then  $W'_1[0:191][8:15]$ then $W'_2[0:191][16:23]$ then $W'_3[0:191][24:31]$ the do output buffer write out, we will need to send with the sequence of $W'_0[0:63][0:7],\; W'_1[0:63][0:7],\; W'_2[0:63][0:7],\; W'_3[0:63][0:7]$, (do memory write out), $W'_0[64:127][0:7],\; W'_1[64:127][0:7],\; W'_2[64:127][0:7],\; W'_3[64:127][0:7]$, (do memory write out), $W'_0[128:191][0:7],\; W'_1[128:191][0:7],\; W'_2[128:191][0:7],\; W'_3[128:191][0:7]$, (do memory write out). After closer examination, this will have minimal impact on THD improvement. Comparing two cases, the only possible extra bit flipping happen when we switch among different sub-matrices; i.e., $W'_0[63][0:7]\rightarrow W'_1[0][0:7],\; W'_1[63][0:7]\rightarrow W'_2[0][0:7],\; W'_2[63][0:7]\rightarrow W'_3[0][0:7],\; W'_3[63][0:7]\rightarrow W'_0[64][0:7],\; W'_0[127][0:7]\rightarrow  W'_1[64][0:7],\; W'_1[127][0:7]\rightarrow W'_2[64][0:7],\; W'_2[127][0:7]\rightarrow W'_3[64][0:7],\; W'_3[127][0:7]\rightarrow W'_0[128][0:7],\; W'_0[191][0:7]\rightarrow W'_1[128][0:7],\; W'_0[191][0:7]\rightarrow W'_1[128][0:7],\; W'_1[191][0:7]\rightarrow W'_2[128][0:7],\; W'_2[191][0:7]\rightarrow W'_3[128][0:7]$. With output buffer depth of $d$, the extra bit flipping happens once after sending sequence length of d, and Hamming Distance overhead will be $\frac{1}{d}$. For reasonable d (e.g. 64 or 128), this overhead is less than 2\%.
\end{example}

Unlike STOSG, C clustering proposed in Section \ref{subsec:c_clustering} does not involve partial sum address issue. C clustering is essentially a dual process of output channel reordering, where output reordering reorders rows of weight matrix and C clustering reorders columns of weight matrix. This means that C clustering will only influence the memory fetching of input activation, but no hardware overhead is involved.

\label{sec:hardware_support}




\begin{table}[ht]
    \centering
    \begin{tabular}{l|cccc}
        \hline
        $\lambda$          & Top-1 Accuracy & Top-5 Accuracy & HD \\
        \hline \hline
        $0.0$               & 94.38          & 99.82         &           \\
        $1 \times 10^{-4}$  & 94.22          & 99.00         &           \\
        \hline
    \end{tabular}
    \caption{}
    \label{tab:cifar10_exp}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|cccc}
        \hline
        $\lambda$          & Top-1 Accuracy & Top-5 Accuracy & HD \\
        \hline \hline
        $0.0$              & 78.21          & 94.53          & \\
        $1 \times 10^{-5}$ & 77.98          & 94.20          & \\
        $3 \times 10^{-5}$ & 77.47          & 94.07          & \\
        $5 \times 10^{-5}$ & 77.29          & 94.24          & \\
        $7 \times 10^{-5}$ & 77.62          & 94.26          & \\
        \hline
    \end{tabular}
    \caption{}
    \label{tab:cifar100_exp}
\end{table}


\subsection{Evaluation Methodology and Results}
We trained MobileNet V2 neural networks on CIFAR100 dataset with various $\lambda_2$ of HDAT to validate our proposed methods. The performance of each neural network is summaries in Table \ref{tab:imagenet_mbnt}.

Then we evaluated the energy consumption in post-layout simulation. We designed an input-stationary systolic array with 8 rows and 2 columns, each PE can support 8-bit (input activation) x 4-bit (weight) multiplication and accumulation. The array is synthesized using Design Compiler and place route using IC CompilerII with TSMC 7nm ULVT technology and energy consumption is evaluated using Prime Time PX. Since pre-loaded input activation data also have an effect on average array energy consumption (for example, if the pre-loaded activation data is 0 then the multiplier energy is the same regardless of weight sequence), we report the average energy over all possible activation cases. In other words, with one weight input sequence, we first set 8-bit preloaded activation data as 1, go through the whole weight sequence, then change preloaded activation data to 2, go through the whole weight sequence again, until we exhaust all possible preloaded activations (255 possibilities in total), and report average energy per operation. Leakage energy is two-orders of magnitude smaller and is ignored here. We then compare the the THD and normalized energy efficiency (operation per unit enery, OP/J) of different versions of neural network over various layers with and without STOSG, as shown in Fig. \ref{fig:baseline_1_THD} - Fig. \ref{fig:baseline_7}. We also summarize the best case and average improvements brought by STOGS and HDAT over various layers in Table~\ref{table-improvement-summary}. 

\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_1_THD.png}
    \caption{THD, baseline vs. $\lambda_2=1e-5$}
    \label{fig:baseline_1_THD}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_3_THD.png}
    \caption{THD, baseline vs. $\lambda_2=3e-5$}
    \label{fig:baseline_3_THD}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_5_THD.png}
    \caption{THD, baseline vs. $\lambda_2=5e-5$}
    \label{fig:baseline_5_THD}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_7_THD.png}
    \caption{THD, baseline vs. $\lambda_2=7e-5$}
    \label{fig:baseline_7_THD}
\end{figure}

\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_1.png}
    \caption{Normalized OP/J, baseline vs. $\lambda_2=1e-5$}
    \label{fig:baseline_1}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_3.png}
    \caption{Normalized OP/J, baseline vs. $\lambda_2=3e-5$}
    \label{fig:baseline_3}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_5.png}
    \caption{Normalized OP/J, baseline vs. $\lambda_2=5e-5$}
    \label{fig:baseline_5}
\end{figure}
\begin{figure}[htp]
    \centering
    \includegraphics[width=\linewidth]{figs/baseline_7.png}
    \caption{Normalized OP/J, baseline vs. $\lambda_2=7e-5$}
    \label{fig:baseline_7}
\end{figure}

%With HDAT only, the best/average energy improvement are 2.16X/1.23X for $\lambda_2=1e-5$, 2.16X/1.23X for $\lambda_2=3e-5$, 4.87X/1.72X for $\lambda_2=5e-5$ and 4.80X/1.81X for $\lambda_2=7e-5$. With STOGS only the best/average THD improvement is 2.42X/1.9X, and the best/average energy improvement is 1.79X/1.54X. By combining HDAT and STOGS, the best/average energy improvement are 2.65X/1.71X for $\lambda_2=1e-5$, 3.92X/2.04X for $\lambda_2=3e-5$, 5.69X/2.47X for $\lambda_2=5e-5$ and 6.98X/2.79X for $\lambda_2=7e-5$. 

\begin{table*}[t]
\caption{THD/Energy Improvement with Proposed Methods.}
\label{table-improvement-summary}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{m{2cm}| m{2cm}| m{2cm}| m{2cm}| m{2cm}}
%\begin{tabular}{l c c c c c c r}
\toprule
Optimization Used & Best THD Improvement & Avg. THD Improvement & Best Energy Improvement & Avg. Energy Improvement \\        
\midrule
STOGS                       &2.42X      & 1.90X     &1.94X       &1.58X\\
HDAT, $\lambda=1e-5$         &2.31X      & 1.24X     &2.17X       &1.26X\\
HDAT, $\lambda=3e-5$         &3.19X      &1.50X      &2.86X       &1.47X\\
HDAT, $\lambda=5e-5$         &4.54X      &1.76X      &3.88X       &1.67X\\
HDAT, $\lambda=7e-5$         &5.95X      &2.00X      &4.92X       &1.86X\\
STOGS+HDAT, $\lambda=1e-5$   &3.31X      &2.10X      &2.65X       &1.76X\\
STOGS+HDAT, $\lambda=3e-5$   &5.33X      &2.57X      &4.10X       &2.09X\\
STOGS+HDAT, $\lambda=5e-5$   &7.98X      &3.15X      &5.69X       &2.47X\\
STOGS+HDAT, $\lambda=7e-5$   &10.19X     &3.68X      &6.98X       &2.79X\\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}



While $W v = W^{\prime\prime} v$, the bit flips of the weight sequence for $W^{\prime\prime}$ is $12$ smaller compared to $W$. 

We observe that if we change the sequence of streaming the weight matrix by swapping along the matrix column direction, i.e., the output channel direction of the convolution, we are able to reduce the bit flips. Consider $W$ in the example above. If we swap the second row and the third row of the matrix, we have $W^{\prime\prime}$ as below:
\begin{equation*}
    W^{\prime} = 
    \left[\begin{array}{cccc}
    00  & 00  & 00 & 00 \\
    \rowcolor{black!20}
    00  & 00  & 00 & 00 \\
    \rowcolor{black!20}
    11 & 11 & 11 & 11 \\
    11 & 11 & 11 & 11
    \end{array}\right]
\end{equation*}
Now, by streaming $W^{\prime}$ into the compute array, the bit flips can be reduced to from $24$ to $8$. \textsl{Note that swapping the rows of the weight matrix is essentially adjusting the order of generating output channels and there is no influence in terms of neural network functionality. As the swapping can be finished via post-processing in model level, no specific hardware support is needed.}

Although the sequence of streaming weight depends on the dataflow, the above observation can be generally applied once the weight matrices are streamed into the arithmetic computation array. Meanwhile, while the bit flips and the sequence of other input operands, e.g., input activations or partial sums, also impact the datapath energy, it is hard to explore similar swapping techniques as these operands are input dependent and thus, cannot be determined a priori during the compile time.

In coding theory, the bit flips of the weight sequence is defined as the hamming distance. 

Without loss of generality, we assume the weights are quantized to 2 bits and are streamed into the input-stationary compute array following Figure~\subref*{fig:1x1_mapping}. Then, the sequence of weights streamed into the first row of the compute array are $\{00, 11, 00, 11\}$ and the bit flips at the compute array input are 6. 

and the bit flips of the weight sequence 
\pierce{mention wihout loss of generality 2 times here. perhaps can just say Consider the example of the following two 2-bit weight matrices?}\meng{Sure}
Consider the example of the following two weight matrices $W, W^\prime \in \mathbb{R}^{K \times C}$:
\begin{align*}
    W & = \left.\left[ 
        \vphantom{\begin{array}{c}1\\1\\1\\1\end{array}}
        \smash{
        \underbrace{
        \begin{array}{cccc}
            00 & 00 & 00 & 00 \\
            11 & 11 & 11 & 11 \\
            00 & 00 & 00 & 00 \\
            11 & 11 & 11 & 11
        \end{array} 
        }_{\textcolor{blue}{C}}
        }
        \right]\right\}
        \,\textcolor{blue}{K}, \\[10pt]
    W^\prime & = \left[ 
        \begin{array}{cccc}
        00 & 11 & 00 & 11 \\
        00 & 11 & 00 & 11 \\
        11 & 00 & 11 & 00 \\
        11 & 00 & 11 & 00
        \end{array} \right].
\end{align*}
%Without loss of generality, we assume multiplication is based on 2-bit operands. If we follow Figure \ref{fig:1x1_example} and stream $W$ and $W^\prime$ into the PE array, then the bit flips for each multiplier become 24 and 8, respectively. We synthesize the design in Figure \ref{fig:is} and find that the datapath energy of streaming $W$ is roughly XXX larger than streaming $W^\prime$. To further confirm the relation between the bit flips and the datapath energy, we generated random data pattern into a systolic array and evaluate energy consumption of various data pattern with post-layout simulation (see Section \ref{sec:results} for detailed experiment setup). As shown in Figure \ref{}, the total bit flips and the energy consumption demonstrate strong linear relation. Moreover, given a certain total bit flips, the energy is independent of the length of the weight sequence and bit flipping probability.
% Without loss of generality, we assume multiplication is based on 2-bit operands. 
Without loss of generality, we assume the weights are quantized to 2 bits. If we follow Figure \ref{fig:1x1_example} and stream $W$ and $W^\prime$ into the PE array, then the number of bit flips for each multiplier become 24 and 8, respectively. 

To confirm the relation between the bit flips and the datapath energy, we generated random data into the compute array and evaluated energy consumption with post-layout simulation (see Section \ref{sec:results} for detailed experiment setup). As shown in Figure \ref{fig:THD_energy}, the total bit flips and the energy consumption demonstrate a strong linear relation. Moreover, given a fixed total bit flips, the energy is independent of the length of the weight sequence and the bit flipping probability.
\yilei{Maybe we should say "Normalized Energy" in y-axis of Figure \ref{fig:THD_energy}}
\meng{I feel "normalized energy" is vague as it is unclear what the denominator should be.}
\vikas{I see Yilei's point. Right now it is unclear what the units are for the y-axis...}

%\meng{Need to mention that directly streaming the weights, the bit flip probability is close to 50\%.}
%This is mentioned in discussion section

Besides the relation between the bit flips and the datapath energy, we also notice that if we change the sequence of streaming the weight matrix by swapping along the matrix column direction, i.e., the output channel direction of the convolution, we are able to reduce the bit flips. Consider $W$ in the example above. If we swap the second row and the third row of the matrix, we have $W^{\prime\prime}$ as below:
\begin{equation*}
    W^{\prime\prime} = 
    \left[\begin{array}{cccc}
    00  & 00  & 00 & 00 \\
    \rowcolor{black!20}
    00  & 00  & 00 & 00 \\
    \rowcolor{black!20}
    11 & 11 & 11 & 11 \\
    11 & 11 & 11 & 11
    \end{array}\right]
\end{equation*}
Now, by streaming $W^{\prime\prime}$ into the compute array, the bit flips can be reduced to from $24$ to $8$. \textsl{Note that swapping the rows of the weight matrix is essentially adjusting the order of generating output channels and there is no influence in terms of neural network functionality. As the swapping can be finished via post-processing in model level, no specific hardware support is needed.}

Although the sequence of streaming weight depends on the dataflow, the above observation can be generally applied once the weight matrices are streamed into the arithmetic computation array. Meanwhile, while the bit flips and the sequence of other input operands, e.g., input activations or partial sums, also impact the datapath energy, it is hard to explore similar swapping techniques as these operands are input dependent and thus, cannot be determined a priori during the compile time.
% Without loss of generality, in this paper, we always use the input stationary dataflow as an example to explain the key concepts and our algorithms.  


==> doc/c_clustering.tex <==
% \section{C Clustering}

\begin{figure}[ht]
    \centering
    \subfloat[]{\includegraphics[width=0.9\linewidth]{figs/motivating_example_array}\label{fig:motivating_array}} \\
    \subfloat[]{\includegraphics[height=0.35\linewidth]{figs/motivating_example_k_swap}\label{fig:motivating_k_swap}}
    \hspace{20pt}
    \subfloat[]{\includegraphics[height=0.35\linewidth]{figs/motivating_example_c_cluster}\label{fig:motivating_c_cluster}}
    \caption{Motivating example: (a) streaming weight matrices into an input stationary PE array; (b) for small weight matrices, re-ordering the sequence of output channels help reduce the total bit flips; (c) for large weight matrices, input channels can be first clustered before feeding into the PE array to further reduce the total bit flips.}
    \label{fig:motivating}
\end{figure}

As shown in Figure \ref{fig:motivating}, when the number of input channel is large, the weight matrices need to be tiled along the $C$ dimension. This provides us with opportunities to further reduce the bit flips (and data path energy) as
\begin{itemize}
    \item The final outcome is not impacted by the order of the input channels and thus, we can cluster different input channels before streaming the weights into the PE array.
    \item For different input channel clusters, the sequence of output channels feeding into the compute array can be different.
\end{itemize}
To formalize the clustering process, let $W \in \mathbb{R}^{k \times c}$ be the network parameters for a layer. The goal is to partition the $c$ input channels into $t$ sets $T = \{T_1, \ldots, T_t\}$ to minimize the within-cluster THD. Let $S = \{S_1, \ldots, S_t\}$ denotes the optimal sequence of output channels for each set. Then, the objective can be formalized as 
\begin{align*}
    \min_{T} \quad & \sum_{i=1}^{t} d_i \\
    \mathrm{s.t.} \quad & d_i = \min_{S_i} \sum_{l=1}^{|T_i|} \sum_{j=1}^{k} \THD(W[S_i[j], l], W[S_i[j+1], l])
\end{align*}
To solve the above optimization problem optimally is NP hard. Hence, we propose a greedy iterative method to solve the nested optimization problem. As shown in Algorithm \ref{alg: c_clustering}, in the initialization process, $t$ input channels are randomly selected and $\{S_1^{(0)}, \ldots, S_t^{(0)}\}$ are initialized to minimize the total hamming distance for each input channel. Then, the algorithm proceeds by alternating between the assignment step and the update step for $N$ total iterations. In the assignment step, for each input channel $i$, we evaluate its THD following the optimal sequence of each cluster and add the channel to the cluster with the smallest THD. In the update step, we re-compute the optimal sequence for each cluster of input channels.

\begin{algorithm}[htb]
\SetAlgoLined
$\{S_1^{(0)}, \ldots, S_t^{(0)}\}, n \leftarrow$ \textsc{Random\_Initialize}(), 0\;
\While{$n \leq N$}{
    \textcolor{blue}{\tcp{Assignment step}}
    \For{$i = 1: c$}{
        $l \leftarrow \argmin_{t} \sum_{j=1}^{k} \THD(W[S_t^{(n)}[j], i], W[S_t^{(n)}[j + 1], i])$\;
        $T_l^{(n)} \leftarrow T_l^{(n)} \bigcup \{i\}$\;
    }
    \textcolor{blue}{\tcp{Update step}}
    \For{$i = 1: t$}{
        $S_i^{(n + 1)} \leftarrow \argmin_{S_i} \sum_{l=1}^{|T_i^{(n)}|} \sum_{j=1}^{k} \THD(W[S_i[j], l], W[S_i[j+1], l])$\; 
    }
    $n += 1$\;
}
\caption{C Clustering}
\label{alg: c_clustering}
\end{algorithm}

The convergence of the clustering algorithm can be guaranteed and the objective can be reduced monotonically if the update step can be optimally solved. However, as mentioned in Section \ref{}, the update step involves an NP-hard problem and hence, we use the greedy algorithm in Algorithm \ref{} to solve the update step, the complexity of which is $O(k^2 c)$. The complexity of the assignment step is $O(ckt)$.

In practice, the number of input channel clusters is determined by the number of input channels and the dimension of the systolic array. Meanwhile, the size of each cluster is limited by the dimension of the systolic array as well. 


==> doc/experiments_bk.tex <==
\onecolumn
\section{Experimental Results}

\begin{itemize}
    \item Cifar10:
    \begin{itemize}
        \item MobileNetV2
        \begin{itemize}
            \item 8-bit weight and 32-bit activation: top-1 accuracy 94.97\%, and top-5 accuracy 99.82, fblearner ID: \% 
            \item 4-bit weight and 32-bit activation: top-1 accuracy 94.84\%, and top-5 accuracy 99.87, fblearner ID: \%
            \item When we add regularization to the 1x1 convolutions:
            \begin{itemize}
                \item $\lambda = 0.0001$, top-1 accuracy 94.22\%, and top-5 accuracy 99.90\%, fblearner ID: f130621963
            \end{itemize}
        \end{itemize}
        \item ResNet56
    \end{itemize}
    \item Cifar100:
    \begin{itemize}
        \item MobileNetV2
        \begin{itemize}
            \item 4-bit weight and 32-bit activation: top-1 accuracy 78.21\%, and top-5 accuracy 94.53\%, fblearner ID: f130753124
            \item 8-bit weight and 32-bit activation: top-1 accuracy 78.06\%, and top-5 accuracy 94.66\%, fblearner ID: f131160194
            \item When we add regularization to the 1x1 convolutions:
            \begin{itemize}
                \item $\lambda = 10^{-6}$, top-1 accuracy 78.04\%, top-5 accuracy 94.09\%, fblearner ID: f130909248
                \item $\lambda = 5 \times 10^{-6}$, top-1 accuracy 77.23\%, top-5 accuracy 93.98\%, fblearner ID: f131029952
                \item $\lambda = 10^{-5}$, top-1 accuracy 76.43\%, top-5 accuracy 93.79\%, fblearner ID: f130909035
            \end{itemize}
        \end{itemize}
        \item ResNet56
    \end{itemize}
    \item ImageNet:
    \begin{itemize}
        \item MobileNetV2
    \end{itemize}
    \item Only add regularization to large layers (in terms of \# FLOPs)
    \begin{itemize}
        \item For MobileNetV2, $FLOPS > 3 \times 10^6$
    \end{itemize}
    \item Pareto front for Cifar100 and MobileNetV2
    \item Impact of bitwidth on the effectiveness: use Cifar100 and MobileNetV2 as an example, use 2-bit, 4-bit and 8-bit
    \begin{itemize}
        \item 
    \end{itemize}
\end{itemize}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$   & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline           
        $0.0$               & 94.38          & 99.82          &          &           & f130350422 \\
        $1 \times 10^{-4}$  & 94.22          & 99.00          &          &           & f130350422 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar10 with MobileNetV2: 4-bit weight}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline           
        $0.0$               & 78.21          & 94.53          & 0.494    &           & f130753124 \\
        $1 \times 10^{-6}$  & 78.04          & 94.09          & 0.424    &           & f130909248 \\
        $5 \times 10^{-6}$  & 77.23          & 93.98          & 0.394    &           & f131029952 \\
        $1 \times 10^{-5}$  & 76.43          & 93.79          & 0.361    &           & f130909035 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2: 4-bit weight}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{ll|ccccc}
        \hline
        $\lambda$           & thres           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline           
        $1 \times 10^{-5}$  & 0               & 76.43          & 93.79          & 0.361    &           & f130909035 \\
        $1 \times 10^{-5}$  & $2 \times 10^6$ & 76.43          & 93.51          & 0.365    &           & f131352902 \\
        $1 \times 10^{-5}$  & $4 \times 10^6$ & 76.95          & 94.30          & 0.387    &           & f131353265 \\
        $1 \times 10^{-5}$  & $8 \times 10^6$ & 77.21          & 93.79          & 0.404    &           & f131353635 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2 (4-bit weight): only add regularization for layers with \# FLOPs larger than the threshold.}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        thres           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline
        0               & 76.43          & 93.79          & 0.361    &           & f130909035 \\
        $2 \times 10^6$ & 76.93          & 93.73          & 0.365    &           & f131508000 \\
        $4 \times 10^6$ & 77.30          & 93.85          & 0.376    &           & f131507363 \\
        $8 \times 10^6$ & 76.97          & 93.95          & 0.386    &           & f131506974 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2 (4-bit weight): for layers with \# FLOPs larger than the threshold, $\lambda = 1 \times 10^{-5}$ and for other layers, $\lambda = 1 \times 10^{-6}$.}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        thres           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline
        0               & 76.43          & 93.79          & 0.361    &           & f130909035 \\
        $2 \times 10^6$ & 77.04          & 94.06          & 0.362    &           & f131640855 \\
        $4 \times 10^6$ & 77.27          & 94.09          & 0.367    &           & f131641318 \\
        $8 \times 10^6$ & 77.29          & 94.10          & 0.368    &           & f131641826 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2 (4-bit weight): for layers with \# FLOPs larger than the threshold, $\lambda = 1 \times 10^{-5}$ and for other layers, $\lambda = 1 \times 5 \times 10^{-6}$.}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$       & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline
        $0.0$              & 78.21          & 94.53          & 0.494    &           & f130753124 \\
        $1 \times 10^{-5}$ & 77.77          & 94.28          & 0.340    &           & f131677608 \\
        $3 \times 10^{-5}$ & 77.34          & 94.20          & 0.232    &           & f131921585 \\
        $5 \times 10^{-5}$ & 77.20          & 94.00          & 0.194    &           & f131677832 \\
        $7 \times 10^{-5}$ & 77.09          & 93.92          & 0.169    &           & f131921754 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2 (4-bit weight): add regularization to layer with expRatio larger than 3.}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$       & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline
        $0.0$              & 78.21          & 94.53          & 0.494    &           & f130753124 \\
        $1 \times 10^{-5}$ & 77.47          & 94.04          & 0.340    &           & f131962438 \\
        $5 \times 10^{-5}$ & 77.08          & 93.87          & 0.193    &           & f131962173 \\
        $1 \times 10^{-4}$ & 76.92          & 94.07          & 0.137    &           & f131962564 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2 (4-bit weight): add regularization to layer with expRatio larger than 3 and output channel larger than 192.}
    \label{tab:imagenet_mbv1}
\end{table}


\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$       & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline
        $0.0$              & 78.21          & 94.53          & 0.494    &           & f130753124 \\
        $1 \times 10^{-5}$ & 77.98          & 94.20          & 0.343    &           & f133466843 \\
        $3 \times 10^{-5}$ & 77.47          & 94.07          & 0.240    &           & f133468142 \\
        $5 \times 10^{-5}$ & 77.29          & 94.24          & 0.196    &           & f133468054 \\
        $7 \times 10^{-5}$ & 77.62          & 94.26          & 0.167    &           & f133468224 \\
        \hline
    \end{tabular}
    \caption{Results on Cifar100 with MobileNetV2 (4-bit weight): add regularization to layer with expRatio larger than 3 and output channel larger than 192 and reorder every 50 epochs.}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline       
        $0$                 & 69.69          & 91.16          & 0.497    &           & f131344452 \\
        $1 \times 10 ^{-3}$ & 54.85          & 84.29          & 0.248    &           & f131345152 \\
        $1 \times 10 ^{-4}$ & 68.13          & 90.93          & 0.403    &           & f131344548 \\
        $5 \times 10 ^{-5}$ & 69.00          & 90.62          & 0.426    &           & f131587985 \\
        $1 \times 10 ^{-5}$ & 69.75          & 90.95          & 0.477    &           & f131344486 \\
        \hline
    \end{tabular}
    \caption{Results on cifar100 with ResNet26 (4-bit weight).}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline       
        $0$                 & 72.00     & 91.38     & 0.497    &           & f131665305 \\
        $1 \times 10 ^{-4}$ & 70.14     & 90.50     & 0.403    &           & f131665393 \\
        $1 \times 10 ^{-5}$ & 72.14     & 91.69     & 0.473    &           & f131665472 \\
        \hline
    \end{tabular}
    \caption{Results on cifar100 with ResNet50 (4-bit weight).}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline       
        $0$                 & 71.93          & 90.20          & 0.499    &           & f131127178 \\
        $1 \times 10^{-7}$  & 71.67          & 90.14          & 0.498    &           & f131132465 \\
        $1 \times 10^{-6}$  & 71.73          & 90.39          & 0.485    &           & f131130398 \\
        $5 \times 10^{-6}$  & 71.19          & 89.96          & 0.447    &           &  f131130689 \\
        $1 \times 10^{-5}$  & 70.55          & 89.62          & 0.427    &           & f131130514 \\
        \hline
    \end{tabular}
    \caption{Results on ImageNet with MobileNetV2 (8-bit weight).}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$           & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline       
        $0$                 & 71.11          & 89.90          & 0.497    &           & f131131258 \\
        $1 \times 10^{-6}$  & 71.14          & 89.94          & 0.483    &           & f131131359 \\
        \hline
    \end{tabular}
    \caption{Results on ImageNet with MobileNetV2 (4-bit weight).}
    \label{tab:imagenet_mbv1}
\end{table}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|ccccc}
        \hline
        $\lambda$       & Top-1 Accuracy & Top-5 Accuracy & Bit Flip & Greedy Opt & Fblearner ID\\
        \hline \hline
        $0.0$              & 71.93          & 90.20          & 0.499    &           & f131127178 \\
        $1 \times 10^{-5}$ & 70.93          & 89.80          & 0.436    &           & f132926458 \\
        $2 \times 10^{-5}$ & 70.04          & 89.24          & 0.431    &           & f132927279 \\
        $8 \times 10^{-6}$ & 71.03          & 84.85          & 0.441    &           & f132927461 \\
        $6 \times 10^{-6}$ & 71.43          & 90.21          & 0.448    &           & f132927495 \\
        \hline
    \end{tabular}
    \caption{Results on ImageNet with MobileNetV2 (8-bit weight): add regularization to layer with expRatio larger than 3 and output channel larger than 192.}
    \label{tab:imagenet_mbv1}
\end{table}


==> doc/hd_aware_training.tex <==
% \section{HD-Aware NN Training}
% \label{sec:hd_aware_training}

To formalize the proposed THD-aware training procedure, consider a $d$-layer neural network and let $W = \{w_i\}_{i=0}^{d-1}$ be the network parameters. For the $i$th layer, suppose $w_i \in \mathbb{R}^{K_i \times C_i}$, where $K_i$ denotes the number of filters and $C_i$ denotes the number of parameters for each filter. For a given sequence of output channels, denoted as $s$, we define the THD-loss as below:
\begin{align*}
    \gL_{THD}(w_i) & = \sum_{j=0}^{K - 2} \THD(w_i[s_j, :], w_i[s_{j + 1}, :]) \\
                        & = \sum_{j=0}^{K - 2} \sum_{b=0}^{B-1} (2 \cdot \Bit_b(w_i[s_j, :]) - 1) \cdot (2 \cdot \Bit_b(w_i[s_{j + 1}, :] - 1)
\end{align*}
where $\Bit_b(w_i[s_j, :]) = \frac{1}{2^b} \floor(w_i[s_j, :] - 2^{b+1} \floor(\frac{1}{2^{b+1}}w_i[s_j, :]))$ computes the $b$th bit for the parameters.

The main problem with $\gL_{THD}$ is that $\floor(\cdot)$ is not differentiable. Previously, STE has been proposed to approximate the gradients. However, STE cannot be directly applied to the $\floor(\cdot)$ function as 
\begin{align*}
    \frac{\partial \Bit_b}{\partial w_i} = 0 \quad \forall b \neq B - 1.
\end{align*}
This indicates only the most significant bit of the weight parameters are regularized and is equivalent to regularizing the magnitude of the weights.

To resolve the problem of STE, we propose an iterative freeze-and-regularize procedure. In the neural network training process, we first add regularization to the most significant bit and after several epochs, we freeze the most significant bit and then, regularize the second most significant bit. The iterative process continues until we fix all the bits of the model. 

The second problem with $\gL_{THD}$ is that the optimal sequence of output channels $s$ is unknown and changes in the training process. For a given weight matrix, searching for the optimal sequence of output channels $s$ can be formulated as a traveling salesman problem, which can be solved approximately with a greedy algorithm. Meanwhile, although $s$ may change as the weights get updated after each batch in the training, we propose to update $s$ only after each epoch to reduce the training time.

Finally, We incorporate the THD loss of the network parameters into the normal loss function by multiplying a scaling factor ($\lambda_2 > 0$), which controls the trade-off between accuracy and the bit flip probability. The final loss function is given as 
\begin{align*}
    \gL = \gL_{CE} + \lambda_1 \sum_{i=0}^{d} || w_i ||_2^2 + \lambda_2 \sum_{i=0}^{d} \gL_{HD}(w_i)
\end{align*}
where $\gL_{CE}$ represents the original cross-entropy loss widely used in the classification problem and $|| w_i ||_2^2$ denotes the weight decay regularization.

The whole training process is now illustrated in Figure \ref{fig:framework}. For each batch, we leverage the fake quantization techniques to quantize the network and then, compute the overall loss function to update the model parameters. After each epoch, we update the output channel order and after a pre-defined number of epochs, we fix the MSB and start to regularize the next bit.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/hd_aware_training.pdf}
    \caption{Overall framework.}
    \label{fig:framework}
\end{figure}

==> doc/meng_draft.tex <==
Overall flow

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\linewidth]{figs/overall_flow.pdf}
    \caption{Overall framework.}
    \label{fig:framework}
\end{figure}

Output stationary dataflow:

\begin{figure}[H]
    \centering
    \subfloat[]{\includegraphics[width=0.3\linewidth]{figs/output_stationary_HW}\label{fig:os_hw}}
    \hspace{30pt}
    \subfloat[]{\includegraphics[width=0.3\linewidth]{figs/output_stationary_HWK}\label{fig:os_hwk}}
    \caption{Output stationary dataflow variants.}
    \label{fig:os}
\end{figure}

Input stationary dataflow:

\begin{figure}[H]
    \centering
    \includegraphics[width=0.3\linewidth]{figs/input_stationary_HWC.pdf}
    \caption{Input stationary dataflow.}
    \label{fig:is}
\end{figure}

Motivating examples:

\begin{figure}[H]
    \centering
    \subfloat[]{\includegraphics[width=0.7\linewidth]{figs/motivating_example_array}\label{fig:motivating_array}} \\
    \subfloat[]{\includegraphics[height=0.25\linewidth]{figs/motivating_example_k_swap}\label{fig:motivating_k_swap}}
    \hspace{20pt}
    \subfloat[]{\includegraphics[height=0.25\linewidth]{figs/motivating_example_c_cluster}\label{fig:motivating_c_cluster}}
\end{figure}

C clustering:

As shown in Figure \ref{}, when $C$ is large, the weight matrices need to be tiled along the $C$ dimension. For different $C$ tiles, the sequence of output channels feeding into the compute array can be different. Because changing the order of input channels does not impact the final outcome, we propose to cluster different input channels first before reordering the output channels.



HD-Aware Training:

Besides the post-training techniques, to further reduce the HD of the weight matrices, we propose to incorporate the HD loss in the network training procedure by adding an extra regularization term to the loss function. 

Consider a $d$-layer neural network and let $\Theta = \{\theta_i\}_{i=0}^{d-1}$ be the network parameters. For the $i$th layer, suppose $\theta_i \in \mathbb{R}^{K_i \times C_i}$, where $K_i$ denotes the number of filters and $C_i$ denotes the number of parameters for each filter. For a given sequence of output channels, denoted as $s$, the HD-loss becomes

\begin{align*}
    \gL_{HD}(\theta_i) & = \sum_{j=0}^{K - 2} \HD(\theta_i[s_j, :], \theta_i[s_{j + 1}, :]) \\
                       & = \sum_{j=0}^{K - 2} \sum_{b=0}^{B-1} (2 \cdot \Bit_b(\theta_i[s_j, :]) - 1) \cdot (2 \cdot \Bit_b(\theta_i[s_{j + 1}, :] - 1)
\end{align*}
where $\Bit_b(\theta_i[s_j, :]) = \frac{1}{2^b} \floor(\theta_i[s_j, :] - 2^{b+1} \floor(\frac{1}{2^{b+1}}\theta_i[s_j, :]))$ computes the $b$th bit for the parameters.

There are mainly two problems concerning $\gL_{HD}$: 1) $\gL_{HD}$ is not differentiable and 2) optimal sequence of output channels $s$ can change with the updates of the model parameters. To make $\gL_{HD}$ differentiable, we use the straight-through estimator (STE) \cite{} for $\floor(\cdot)$. For the second problem, we find updating $s$ every batch makes the training unstable. Hence, we update $s$ after each epoch of training.

We incorporate the HD loss of the network parameters into the normal loss function by multiplying a scaling factor ($\lambda_2 > 0$), which controls the trade-off between accuracy and the bit flip probability. The final loss function is given as 

\begin{align*}
    \gL = \gL_{CE} + \lambda_1 \sum_{i=0}^{d} || \theta_i ||_2^2 + \lambda_2 \sum_{i=0}^{d} \gL_{HD}(\theta_i)
\end{align*}

The whole training process is now illustrated in Figure \ref{}. For each batch, we leverage the fake quantization techniques proposed in \cite{} to quantize the network and then, compute the overall loss function. STE is exploited to enable backward propagation and model parameter updating. Then, after each epoch, we reorder the output channels based on the current model parameters leveraging Algorithm \ref{}.



==> doc/outline.tex <==
\onecolumn

Introduction:
\begin{itemize}
    \item Motivation
    \begin{itemize}
        \item Accelerator energy breakdown: datapath consumes significant portion of power
        \item Especially with the improvement of near-memory computing, the datapath energy becomes even more significant
    \end{itemize}
    \item Datapath energy = \# OPs $\times$ energy/OP $\times \lambda$
    \begin{itemize}
        \item \# OPs is determined by the model
        \item energy/OP is determined by the hardware, i.e., bit precision
        \item $\lambda$ is hardware factor
    \end{itemize}
    \item Existing researches focus on reducing the first two items. For $\lambda$, only the sparsity of the weights and activations have been exploited. \textit{In the paper, we propose a new dimension to reduce $\lambda$, i.e., hamming distance of weights}
\end{itemize}

Methodology:
\begin{itemize}
    \item Explain why the hamming distance matters
    \begin{itemize}
        \item Explain why HD matters for the accelerators
        \item Without any optimization, the hamming distance of neighboring vectors are close to zero
    \end{itemize}
    \item How to optimize the hamming distance
    \begin{itemize}
        \item Hardware-centric methods:
        \begin{itemize}
            \item $Z_{out}$ swapping
            \begin{itemize}
                \item No hardware overhead
                \item Problem is NP and thus, proposes a greedy method
            \end{itemize}
            \item $Z_{in}$ clustering
            \begin{itemize}
                \item Large $Z_{in}$ is hard to optimize directly
                \item Spatial accelerators only process limited $Z_{in}$ simultaneously
                \item Split/Cluster $Z_{in}$ and use different $Z_{out}$ sequences for different clusters
                \item How to do the clustering: greedy algorithm + convergence proof
                \item Extra hardware support is needed
            \end{itemize}
        \end{itemize}
        
        \item Training-aware methods:
        \begin{itemize}
            \item For a large $Z_{in}$ and $Z_{out}$, hardware-centric methods may not be very effective
            \item Training-aware methods provide the opportunity to optimize the HD in the training process and an extra dimension to trade-off between accuracy and energy
            \item How to add the regularization
        \end{itemize}
    \end{itemize}
\end{itemize}

Experimental results:
\begin{itemize}
    \item Key results:
    \begin{itemize}
        \item Comparison on MobileNetV2 and Cifar10/Cifar100/ImageNet for the following options:
        \begin{itemize}
            \item Baseline with no optimizations
            \item $Z_{out}$ swap only
            \item $Z_{out}$ swap and $Z_{in}$ clustering
            \item Add regularization
        \end{itemize}
    \end{itemize}
    \item Ablation study:
    \begin{itemize}
        \item Impact of $Z_{in}$ and $Z_{out}$
        \item Impact of regularization v.s. accuracy v.s. energy
    \end{itemize}
\end{itemize}
